ZLB: A Blockchain to Tolerate Colluding Majorities

In the general setting, consensus cannot be solved if an adversary controls a third of the system. Yet, blockchain participants typically reach consensus "eventually" despite an adversary controlling a minority of the system. Exceeding this $\frac{1}{3}$ cap is made possible by tolerating transient disagreements, where distinct participants select distinct blocks for the same index, before eventually agreeing to select the same block. Until now, no blockchain could tolerate an attacker controlling a majority of the system. In this paper, we present Zero-Loss Blockchain (ZLB), the first blockchain that tolerates an adversary controlling more than half of the system. ZLB is an open blockchain that combines recent theoretical advances in accountable Byzantine agreement to exclude undeniably deceitful replicas. progressively reduces the portion of deceitful replicas below $\frac{1}{3}$, and reaches consensus. Geo-distributed experiments show that ZLB outperforms HotStuff and is almost as fast as the scalable Red Belly Blockchain that cannot tolerate $n/3$ faults.

==> inc/08application_finalization.tex <==
\subsection{A Zero-Loss Payment Application}\label{ssec:payment}
\label{ssec:eval-payment}


In this section, we describe how \blockchain can be used to implement a \emph{zero-loss payment system} where no honest replica loses any coin.  
%ARPN{I think this next sentence is not making too much sense: (we cannot ask them to deposit huge quantities in order to transfer huge quantities:}
The key idea is to request the consensus replicas to deposit a sufficient amount of coins in order to spend, in case of an attack, the coins of deceitful replicas to avoid any honest replica loss.

 \paragraph{Attacking the SBC solution} In the solution to the SBC problem (Def.~\ref{def:sbc}), deceitful replicas can form a coalition of $f\geq n/3$ replicas to lead honest replicas to a disagreement by \emph{equivocating} (sending distinct messages) to different partitions of honest replicas, with one of two coalition attacks:
%When $f\geq n/3$, disagreement is reached with either one of two attacks: 
\begin{enumerate}[leftmargin=*,wide=\parindent]
\item {\bf Reliable broadcast attack:} deceitful replicas misbehave during the reliable broadcast by sending different proposals to different partitions, leading honest replicas to end up with distinct proposals at the same index $k$. For example, deceitful replicas send block $b_a$ with transaction $tx_a$ to a subset $A$ of honest replicas, while block $b_b$ with conflicting transaction $tx_b$ to a subset $B$ of honest replicas, $A\cap B=\emptyset$, both at the same index $k$. 
\item  {\bf Binary consensus attack:}  deceitful replicas vote for each binary value in each of two partitions for the same binary consensus leading honest replicas to decide different bits in the same index of their bitmask, where deciding $1$ (resp. 0) at bitmask index $k$ means to include (resp. not include) proposal at index $k$ in the Blockchain. For example, deceitful replicas send messages to decide $1$ and $0$ to a subset of honest replicas $A$, while they send messages to decide $0$ and $1$ to a subset $B$ of honest replicas, with $A\cap B=\emptyset$, on the binary consensus instances associated to block $b_a$ with transaction $tx_a$ and block $b_b$ with conflicting transaction $tx_b$, respectively.
\end{enumerate}

Note that deceitful replicas do not benefit from combining these attacks: If two honest replicas deliver different proposals at index $k$, the disagreement comes from them outputting 1 at the corresponding binary consensus instance. Similarly, forcing two honest replicas to disagree during the $k^{\ms{th}}$ binary consensus only makes sense if they both have the same corresponding proposal at index $k$.

 \paragraph{Assumptions}
%\UPDATE{Maybe add (review Vincent): Each transaction carries a strictly increasing sequence number for each user, and it can only be written in the blockchain if the transaction with the previous sequence number is already written. Thus, a double spend requires a user to upload two conflicting transactions with the same sequence number, being such user easily identifiable as taking part in the attack, and its deposit taken to fund such transactions.}\vincent{Added details in section Block Manager}
%\ARPN{I would change it to:}\NEW{In this payment system, replicas hold an amount of voting power directly proportional to the amount of circulating supply they hold (e.g. Proof-of-Stake). 
%The portion of voting power of a replica equals the
%portion of coins that a replica owns in the payment system.
%%
%When attackers are slashed, their funds are moved to the deposit.
In order to measure the expected impact of a coalition attack succeeding with probability $\rho$ 
in forking \blockchain by leading a consensus to disagreement, we first need to make the following assumptions:
\begin{enumerate}[leftmargin=*,wide=\parindent] %[wide, labelwidth=!, labelindent=0pt]
 \item {\bf Fungible assets.}
We assume that users can transfer assets (like coins) that are \emph{fungible} in that one unit is interchangeable and indistinguishable from another of the same value. An example of a fungible asset is a cryptocurrency.
%If assets are not fungible, we assume that there exists a function $\ms{fungibility}:\mathds{D}^a \rightarrow \mathds{C}^{a-1} \times \mathds{D}$ that, given $'a'$ conflicting decisions $d^{P_0},...,d^{P_{a-1}}$, it outputs only one of them $d^{P_r}$ and a list of fungible assets that the rest of the partitions are willing to take as a refund for their decision being forgotten from that instance on. We refer to the function $\ms{fungibility}$ as the \emph{fungibility function}. An example is a replica willing to take the value of a product, if the product was accidentally sent to a different replica. 
% We assume that an honest client does not issue conflicting transactions, i.e., concurrent transactions that withdraw from the same account.
\item {\bf Deposit refund.}
%\ARP{As in classic blockchains~\cite{Nak08,Woo15}, 
%we upper-bound the amount of deposited coins that can be refunded per block.}
  To limit the impact of one successful double spending on a block, \blockchain keeps the deposit for a number of blocks $m$, before returning it. A transaction should not be considered \textit{final} (i.e. irreversible) until it reaches this blockdepth $m$. We call thus $m$ the \textit{finalization blockdepth}. Attackers can fork into $a$ branches, and try to spend multiple times an amount $\mathfrak{G}$ (per block), which we refer to as the \textit{gain}, obtaining a maximum gain of $(a-1)\mathfrak{G}$. 
  Each correct replica can calculate the gain by summing up all the outputs of all transactions in their decided block. Additionally, replicas can limit the gain to an upper-bound by design, discarding blocks whose sum of outputs exceed the bound, or they can allow the gain to be as much as the entire circulating supply of assets. The \textit{deposit} $\mathfrak{D}$ is a factor of the gain, i.e., $\mathfrak{D}= b\cdot \mathfrak{G}$. The goal is for every coalition to have at least $\mathfrak{D}$ deposited, and since every coalition has at least size $\ceil{n/3}$, this means that each replica must deposit an amount $3b\mathfrak{G}/n$.

  
%
%This limit implies that transferring\vincent{or refunding?} a large amount can be done only across $m$ blocks (until the corresponding portion of the deposit is fully refunded) that we refer to as the \emph{depth} of the attack.
%We impose this limit to force a particular amount of coins to take at least a specific amount of blocks $m$ to be transferred entirely, since \blockchain can wrongly decide a transaction $\ms{tx}$ at consensus instance $k$. We denote this value $m$ as the \emph{depth} of an attack. 
%Instead of upper-bounding the amount of coins per block, 
%We can limit $m$ by saying that a transaction $\ms{tx}$ is \emph{confirmed} only when sufficiently many consensus  instances have followed as in classic payment systems~\cite{Nak08,Woo15}.
%We thus assume that $m\geq \frac{a\rho}{1-\rho}$ blocks.
% We show below that we ensure zero loss when $m\geq \frac{a\rho}{1-\rho}$, where $a$ is the number of branches.
%s\NEW{Notice one can instead force $m$ without limiting the coins per block, by delaying confirmation of transactions. Our model also provides a valid $m$ for such simpler approach}.
% are needed in order to confirm a transaction.
 \item {\bf Network control restriction.}
Once faulty replicas select the disjoint subsets (i.e., the partitions) of honest replicas to double spend, 
we need to prevent Byzantine replicas from communicating infinitely faster than honest replicas in different partitions.
%\vincent{What follows does not prevent the two fastest Byzantine replicas from communicating infinitely faster than the two slowest honest replicas.}
%To this end, we assume the ratio of the communication speed of the two fastest honest replicas (from different partitions) over the communication speed of the two slowest Byzantine replicas is upper bounded in expectation. % by $1-\varepsilon$.
%
More formally, let $X_1$ (resp. $X_2$) be the random variables that indicate the time it takes for a message between two replicas within the same partition (resp. two honest replicas from different partitions). We have $E(X_1) / E(X_2) > \varepsilon$, for some $\varepsilon > 0$. Note that the definition of $X_1$ also implies that it is the random variable of the communication time of either two honest replicas of the same partition or two Byzantine replicas. Notice that this probabilistic synchrony assumption is similar to that of Bitcoin and other blockchains that guarantee exponentially fast convergence, a result that also holds for \blockchain under the same assumptions. Notwithstanding, we show in the following an analysis focusing on the attack on each consensus iteration, considering a successful disagreement if there is a fork in a single consensus instance, even for a short period of time. % For simplicity, we consider only identifying each disagreement before it succeeds in a consensus instance, even if \blockchain can detect a disagreement after it took place.
  % \ARPN{Also note that we do not require the specific value of $\epsilon$.}
\end{enumerate}

% \vspace{\skipspace}
\paragraph{Theoretical analysis.}
% \begin{itemize}[wide, labelwidth=!, labelindent=0pt]
% \item{\bf Theoretical analysis}
We show that attackers always fund at least as much as they steal.
We consider that a membership change starts before a disagreement occurs or does not start, which is safer than the general case. Therefore, the attack represents a Bernoulli trial that succeeds with probability $\rho$ (per block) that can be derived from $\varepsilon$.
Out of one attack attempt, the attackers may gain up to $(a-1)\mathfrak{G}$ coins by forking or lose at least $\mathfrak{D}$ coins 
as a punishment from the system. In case of a successful attack, the system compensates the coin losses using the deposited coins. 


We introduce the random variable $Y$ that measures the number of
attempts for an attack to succeed and follows a geometric
distribution with mean $E(Y)=\frac{1-\hat{\rho}}{\hat{\rho}}$, where
$\hat{\rho} = 1 - \rho$ is the probability that the attack fails. Thus, we
define the expected gain of attacking:
\begin{align*}
  \mathcal{G}(\hat{\rho}) =(a-1)\cdot (\mathds{P}(Y>m)\cdot \mathfrak{G})
\end{align*}
and the expected punishment as:
\begin{align*}
  \mathcal{P}(\hat{\rho}) =\mathds{P}(Y\leq m)\cdot \mathfrak{D}
\end{align*}
We can then define the expected \textit{deposit flux} per attack
attempt as the difference
$\Delta=\mathcal{P}(\hat{\rho})-\mathcal{G}(\hat{\rho})$ between the
expected punishment and the expected gain. Theorem~\ref{thm:zeroloss} shows the values for which
\blockchain yields zero-loss.
\begin{theorem}[Zero Loss Payment System]\label{thm:zeroloss}
Let %$f$ the number of deceitful replicas and 
$\rho$ be the probability of success of an attack per block, $\mathfrak{D}$ the minimum deposit per coalition expressed as a factor of the upper-bound on the gain $\mathfrak{D}=b \mathfrak{G}$, and $m$ the finalization blockdepth to return the deposit.
If $g(a,b,\rho,m)=(1-\rho^{m+1})b-(a-1)\rho^{m+1}\geq\,0$ then \blockchain implements a zero loss payment system.
%\blockchain ensures zero loss if the total amount to be transferred in a consensus instance is limited to $\frac{\mathds{C}}{3m}$, where $\mathds{C}$ is the total circulating supply and $m$ is the minimum number of blocks that follow a confirmed transaction.\ARPN{Talk about this theorem: we made $m$ depend on $\rho$ (probability of attack on block succeding). Also, $m$ is actually the number of blocks an attack must last to be precise (in terms of stealing little by little due to the limit of coins per block)}
\end{theorem}
\begin{proof}
Recall that the maximum gain of a successful attack is $\mathfrak{G}
\cdot (a-1)$, and the expected gain $\mathcal{G}(\hat{\rho})$ and punishment $\mathcal{P}(\hat{\rho})$ for the attackers in a
disagreement attempt are as follows:
\begin{align*} \mathcal{G}(\hat{\rho}) =&(a-1)\cdot (\mathds{P}(Y>
m)\cdot \mathfrak{G}) =(a-1)\cdot (\rho^{m+1}\cdot \mathfrak{G}),\\
\mathcal{P}(\hat{\rho}) =&\mathds{P}(Y\leq m)\cdot \mathfrak{D} =
(1-\rho^{m+1})\mathfrak{D}=(1-\rho^{m+1})b\mathfrak{G}.
  \end{align*}

Thus the deposit flux $\Delta=\mathcal{P}(\hat{\rho})-\mathcal{G}(\hat{\rho})$:
$$\Delta=\mathfrak{G}\cdot \bigg((1-\rho^{m+1})b-(a-1)\rho^{m+1}\bigg)\mathfrak{G}=g(a,b,\rho,m)\mathfrak{G}.$$

If $\Delta< 0$ then a cost of $\mathcal{G}(\hat{\rho})-\mathcal{P}(\hat{\rho})$ is incurred to the system, otherwise the punishment is enough to fund the conflicts. Thus, we explore values for which $\Delta\geq 0$. Since the gain is non-negative $\mathfrak{G}\geq 0$, it follows that $g(a,b,\rho,m)\geq 0$ for zero-loss.
\end{proof}

Setting $c=\frac{b}{a-1+b}$, we can either calculate the probability $\rho\leq c^{\frac{1}{m+1}}$ of success for an attack that \blockchain tolerates given a finalization blockdepth $m$, or a needed finalization blockdepth $m\geq \frac{\log(c)}{\log(\rho)}-1$ for a probability $\rho$ to yield zero-loss, once we fix the deposit $\mathfrak{D}$ and upper-bound the gain $\mathfrak{G}$. 
% Under these values that yield $g(a,b,\rho,m)\geq\,0$, we obtain zero-loss, since the remaining deposited funds will always be at least as much as what the attackers manage to steal.

%%%%
 
\paragraph{Simulating the depth and width of a coalition attack.}
% \item{\bf Simulating the depth and width of a coalition attack}
   % Figure~\ref{fig:tap}(left)\CHANGE{this figure can be removed?} indicates the maximum amount of branches $a$ that a coalition of size $f$ can create in a disagreement, for different values of $f$ and $n$.
   % It is specially interesting to observe that a coalition of less than $n/2$ replicas cannot generate more than two branches. 
   % %than a double-disagreement. 
   % % We note the asymptotical limits indicating that, given its size, a coalition cannot create another branch without an additional replica.
   % %We can see that values that are close to a threshold converge asymptotically to breaking the threshold into generating one more branch, but can never do it without one more replica. 
   % Furthermore, Lemma~\ref{lem:011} shows that a deceitful ratio of less than $11/18$
   % can create at most 7 branches per fork.   %while being significantly close, at only $n/18$ of distance, to the threshold value of $2n/3$.
   % %Note that ratio is particularly close to the ratio of $2n/3$.
% \noindent 
Considering a deceitful ratio $\delta=\frac{f-q}{n}$, one can derive the maximum number of branches from the bound $a\leq\frac{n-(f-q)}{\ceil{2n/3}-(f-q)}$~\cite{singh2009zeno}. % Thus, given a deceitful ratio $\delta$, it is possible to estimate the maximum probability of an attack succeeding for a particular depth of an attack, or the other way around. 
For example, for a deceitful ratio of $\delta=0.5,\, a=3$, and for a probability $\rho=0.55$, fixing the depth of the attack to $m=4$ blocks already guarantees zero-loss even if the deposit is a tenth of the maximum gain $\mathfrak{D}=\mathfrak{G}/10$, but increasing $\rho=0.9$ requires to take at least $m=28$ blocks to finish. Whereas $m$ increases polynomially with $\rho$, it increases exponentially as the deceitful ratio $\delta$ approaches the asymptotic limit $2/3$, since the number of branches also increases exponentially fast, with $m=37$ blocks for $\delta=0.6$, while $m=46$ for $\delta=0.64$ or $m=58$ for $\delta=0.66$, with $\rho=0.9$.
% shows the required depth $m$ of an attack for a zero-cost recovery, with variable deceitful ratio $\delta$ and probability $p$. Notice the exponential growth of the depth of attack as the deceitful ratio approaches $\frac{2n}{3}$.} % shows the required amount of consecutive consensus instances $m$ for \blockchain to retrieve enough coins from punishments to fund the block merge.
% The right figure shows the value $m$ per deceitful ratio $\delta$. Notice how $m$ grows linearly with $a$, but exponentially with $\delta$.
 %The right figure shows the value $m$ per deceitful ratio $\delta$. Notice how $m$ grows linearly with $a$, but exponentially with $\delta$. For $\delta \leq 0.6$ (i.e., allowing up to
%%sextuple-disagreement) 
%6 branches per fork) we require $m\geq 54$, even for $\rho=0.9$.
%%\vincent{Explain why the probabilistic result does not contradict our motivations - we can still generate coins out of thin air.}

\begin{figure}[t]
  \hspace{-2em}
  \includegraphics[height=9.5em]{./plots_usenix21/plot_recovery_cost_blockdepth.pdf}
  \caption{Minimum required finalization blockdepth $m$ to obtain zero-loss for $\mathfrak{D}=\mathfrak{G}/10$ and $f=\lceil 5n/9\rceil-1$, per number of replicas %and %different limits on the 
  %maximum amounts $\ell$ of coins 
    `rbbcast' indicates the reliable broadcast attack.%\vincent{It means that if we loose money sometimes, we will gain overall if the size of the system is large enough. We extracted for the blue line the mean deposit flux that depends on l=10\% the percentage of money the coalition can spend in one proposal, given the experiments of Fig.8.}
  }
  \vspace{-1em}
  \label{fig:fig6}
\end{figure}
 
% \vspace{\skipspace}
%\subsection{Evaluation of the Payment System}\label{ssec:eval-payment}
% \paragraph{Experimental evaluation of the payment system.}\label{ssec:eval-payment}

\paragraph{Experimental evaluation of the payment system.}
% \item{\bf Experimental evaluation of the payment system} 
Taking the experimental results of~\cref{sec:expe} and based on our aforementioned theoretical analysis, Figure~\ref{fig:fig6} depicts the minimum required finalization blockdepth $m$ for a variety of uniform communication delays for $\mathfrak{D}=\mathfrak{G}/10$ and %, with $\ell$ being the percentage of total circulating supply allowed to be transferred per proposal and 
$f=\lceil 5n/9\rceil-1$. Again, we can see that the finalization blockdepth decreases with the number of replicas, confirming that the zero loss property scales well. 
Additionally, small uniform delays yield zero loss at smaller values of $m$, with all of them yielding $m<5$ blocks for $n>80$. % Nonetheless, although omitted in the figure, all delays shown lead to $m<10$ for at least 90 replicas with $\ell\leq 50\%$ of the total circulating supply. This means that if \blockchain simply returns half the deposit immediately after deciding a transaction, and the other half after the following block is decided, no honest user will lose any asset whatsoever, even if some attacks succeed.
%
%We can see that for lower uniform delays, the system can allow up to the entire circulating supply to be transferred in one single proposal, since attackers are discovered before they can even cause one disagreement, for an increasing number of replicas, while for really big uniform delays \blockchain needs to lower the value $\ell$ to guarantee the gainful property. 
%
Although omitted in the figure, our experiments showed that even for a uniform delay of 10 seconds, setting $m=50$ blocks (resp. $m=168$ blocks) still yields zero-loss in the case of a binary consensus attack (resp. reliable broadcast attack). 
Nevertheless, if the network performs normally, \blockchain will support large values of $f$, and will actually benefit from attacks (i.e., obtaining more from the deposits than is lost from the attack).

\paragraph{Discussion on probabilistic synchrony}
%\item{\bf Discussion on probabilistic synchrony} 
We assume probabilistic synchrony in this section in order to introduce a probability of failure of an attack per consensus iteration. In partial synchrony, since the committee remains static until fraudsters are identified, the adversary can successfully perform an attack with probability of success $\rho=1$. There are, however, other factors that could influence the probability $\rho$ even in partial synchrony. For example, considering a blockdepth $m\geq 1$, the implementation of a random beacon~\cite{GHM17} that replaces the committee in every iteration can decrease the probability of success of an attack. In such a case, the probability of an attack succeeding depends on the probability that the random beacon selects enough replicas of the coalition (and enough of each of the partitions of correct replicas) for $m+1$ consecutive iterations, so that the coalition is able to perform the attack for $m$ additional blocks. The design and proof of a correct random beacon that tolerates coalitions of sizes greater than $\ceil{n/3}-1$ is part of our future work.

%\end{itemize}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../long-live-blockchain"
%%% End:

